A broken FEEC framework for electromagnetic problems on mapped multipatch domains

We present a framework for the structure-preserving approximation of partial differential equations on mapped multipatch domains, extending the classical theory of finite element exterior calculus (FEEC) to discrete de Rham sequences which are broken, i.e., fully discontinuous across the patch interfaces. Following the Conforming/Nonconforming Galerkin (CONGA) schemes developed in [http://dx.doi.org/10.1090/mcom/3079, arXiv:2109.02553, our approach is based on: (i) the identification of a conforming discrete de Rham sequence with stable commuting projection operators, (ii) the relaxation of the continuity constraints between patches, and (iii) the construction of conforming projections mapping back to the conforming subspaces, allowing to define discrete differentials on the broken sequence. This framework combines the advantages of conforming FEEC discretizations (e.g. commuting projections, discrete duality and Hodge-Helmholtz decompositions) with the data locality and implementation simplicity of interior penalty methods for discontinuous Galerkin discretizations. We apply it to several initial- and boundary-value problems, as well as eigenvalue problems arising in electromagnetics. In each case our formulations are shown to be well posed thanks to an appropriate stabilization of the jumps across the interfaces, and the solutions are extremely robust with respect to the stabilization parameter. Finally we describe a construction using tensor-product splines on mapped cartesian patches, and we detail the associated matrix operators. Our numerical experiments confirm the accuracy and stability of this discrete framework, and they allow us to verify that expected structure-preserving properties such as divergence or harmonic constraints are respected to floating-point accuracy.

==> macros_ppc.tex <==

%\usepackage[right]{showlabels}

%%%%%%%%%%%%  extracting \llangle and \rrangle from MnSymbol package:
\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother
%%%%%%%%%%%%



\usepackage[T3,T1]{fontenc}
\DeclareSymbolFont{tipa}{T3}{cmr}{m}{n}
\DeclareMathAccent{\invbreve}{\mathalpha}{tipa}{16}


% macro: personal comments -- choose your favorite color ;)
\definecolor{darkgreen}{rgb}{.1,.5,0}
\providecommand{\martin}[1]{\textcolor{violet}{(Martin: #1)}}
\providecommand{\eric}[1]{ \textcolor{blue}{Eric: #1}}
\providecommand{\yaman}[1]{\textcolor{darkgreen}{(Yaman: #1)}}



% macro: accent for test functions
\newcommand{\test}[1]{\check{#1}}

% macro: accent for dual complex objects on the logical domain
% \newcommand{\dualhat}[1]{\invbreve{#1}}
\newcommand{\dualhat}[1]{\breve{#1}}



% NOTE on bold fonts: it seems that
% \usepackage[bbgreekl]{mathbbol} is enough,
% > then bbm and bm probably not needed
% \usepackage{bbm}
% \usepackage{bm}  % redefines \boldsymbol for better spacings, see http://tex.stackexchange.com/questions/3238/bm-package-versus-boldsymbol
\def\bs{\boldsymbol}
\def\t{\tilde}
\def\wt{\widetilde}
\def\wh{\widehat}

% Poincaré constants
\def\cp{c_{P}}
\def\cph{c_{P,h}}
\def\bcp{\bar c_{P}}
\newcommand{\poplus}{\overset{\perp}{\oplus}}

\newcommand{\perpW}{{\perp_W}}
\newcommand{\perph}{{\perp_h}}

\def\ext{{\rm ext}}
% \def\frH{\mathfrak{H}}
% \def\frZ{\mathfrak{Z}}
% simple fonts to avoid too many alphabets (for now?)
\def\frB{\mathfrak B}
\def\frH{\mathfrak H}
\def\frZ{\mathfrak Z}

\def\ti{\tilde \imath}
\def\vp{{\varphi}}
\def\ve{{\varepsilon}}
\def\eps{{\epsilon}}

\def\Nppc{N_{\rm ppc}}
\def\pw{{\rm pw}}
\def\ind{{\rm index}}

\def\ba{{\bs a}}
\def\bb{{\bs b}}
\def\bc{{\bs c}}
\def\be{{\bs e}}
\def\bsf{{\bs f}}
\def\bh{{\bs h}}
\def\bi{{\bs i}}
\def\bj{{\bs j}}
\def\bk{{\bs k}}
\def\bsm{{\bs m}}
\def\bn{{\bs n}}
\def\bp{{\bs p}}
\def\bq{{\bs q}}
\def\br{{\bs r}}
\def\bu{{\bs u}}
\def\bv{{\bs v}}
\def\bw{{\bs w}}
\def\bx{{\bs x}}
\def\by{{\bs y}}
\def\bz{{\bs z}}

\def\bA{{\bs A}}
\def\bB{{\bs B}}
\def\bC{{\bs C}}
\def\bD{{\bs D}}
\def\bE{{\bs E}}
\def\bF{{\bs F}}
\def\bG{{\bs G}}
\def\bH{{\bs H}}
\def\bI{{\bs I}}
\def\bJ{{\bs J}}
\def\bK{{\bs K}}
\def\bL{{\bs L}}
\def\bM{{\bs M}}
\def\bN{{\bs N}}
\def\bP{{\bs P}}
\def\bQ{{\bs Q}}
\def\bR{{\bs R}}
\def\bS{{\bs S}}
\def\bV{{\bs V}}
\def\bW{{\bs W}}
\def\bX{{\bs X}}
\def\bY{{\bs Y}}
\def\bZ{{\bs Z}}

\def\bell{{\bs \ell}}
\def\btau{{\bs \tau}}
\def\bvp{{\bs \varphi}}
\def\bpsi{{\bs \psi}}
\def\bnabla{{\bs \nabla}}
\def\bLambda{{\bs \Lambda}}
\def\bGamma{{\bs \Gamma}}


\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}

\def\bfx{{\bf x}}
\def\bfv{{\bf v}}

\def\bfA{{\bf A}}
\def\bfB{{\bf B}}
\def\bfE{{\bf E}}
\def\bfJ{{\bf J}}
\def\bfM{{\bf M}}
\def\bfP{{\bf P}}
\def\bfF{{\bf F}}
\def\bfR{{\bf R}}

\def\bftA{\tilde {\bf A}}
\def\bftC{\tilde {\bf C}}
\def\bftM{\tilde {\bf M}}


% blackboard fonts (eg for number sets)
% \mathbbm, \mathbbmss or \mathbbmtt with \usepackage{bbm}
\def\AA{\mathbbm{A}}
\def\BB{\mathbbm{B}}
\def\CC{\mathbbm{C}}
\def\DD{\mathbbm{D}}
\def\EE{\mathbbm{E}}
\def\FF{\mathbbm{F}}
\def\GG{\mathbbm{G}}
\def\II{\mathbbm{I}}
\def\JJ{\mathbbm{J}}
\def\KK{\mathbbm{K}}
\def\MM{\mathbbm{M}}
\def\NN{\mathbbm{N}}
\def\PP{\mathbbm{P}}
\def\QQ{\mathbbm{Q}}
\def\RR{\mathbbm{R}}
\def\SS{\mathbbm{S}}
\def\TT{\mathbbm{T}}
\def\VV{\mathbbm{V}}
\def\WW{\mathbbm{W}}
\def\XX{\mathbbm{X}}
\def\YY{\mathbbm{Y}}
\def\ZZ{\mathbbm{Z}}
% \def\BB{\mathbb{B}}
% \def\CC{\mathbb{C}}
% \def\DD{\mathbb{D}}
% \def\GG{\mathbb{G}}
% \def\HH{\mathbb{H}}
% \def\II{\mathbb{I}}
% \def\MM{\mathbb{M}}
% \def\NN{\mathbb{N}}
% \def\PP{\mathbb{P}}
% \def\QQ{\mathbb{Q}}
% \def\RR{\mathbb{R}}
% \def\ZZ{\mathbb{Z}}

% % bold blackboard fonts
% % \mathbbm, \mathbbmss or \mathbbmtt with \usepackage{bbm}
% \def\bAA{\mathbbm{A}}
% \def\bCC{\mathbbm{C}}
% \def\bNN{\mathbbm{N}}
% \def\bPP{\mathbbm{P}}
% \def\bRR{\mathbbm{R}}
% \def\bZZ{\mathbbm{Z}}

\def\one{{\mathbbm{1}}}

\def\gl{\mathrm{GL}}

%\usepackage{relsize}
\usepackage{ esint }
\def\fintOm{{\fint_\Omega}}

\def\cNII{\cN^{\rm {II}}}
\def\cNI{\cN^{\rm {I}}}
\def\cRT{\mathcal{RT}}
\def\cBDM{\mathcal{BDM}}

\def\vol{{\rm vol}}
\def\face{{\rm face}}
\def\edge{{\rm edge}}
\def\vertex{{\rm vertex}}
\def\cell{{\rm cell}}

\def\parts{{\rm parts}}

\def\sfA{\mathsf{A}}
\def\sfM{\mathsf{M}}
\def\sfP{\mathsf{P}}
\def\sfT{\mathsf{T}}


\def\Pe{{\sfP^{1}_{h,0}}}
\def\Pm{{\sfP^{0}_h}}

\def\Veh{V^\ve_h}
\def\tVeh{{\t V^\ve_h}}
\def\Vmh{V^\mu_h}
\def\tVmh{{\t V^{\mu}_h}}
\def\Vnuh{V^{\nu}_h}

\def\DG{{\rm DG}}
\def\pFE{{p_{\rm fe}}}
\def\pDG{{p_{\rm dg}}}

\def\intstepn{\int_{t^n}^{t^{n+1}}\mspace{-10mu}}
\def\rmd{\, {\rm d}} %for integrals
\def\dd{\, {\rm d}} %for integrals
\def\Dt{{\Delta t}}
\def\dt{{\partial_{t}}}
\def\dx{{\partial_{x}}}
\def\dy{{\partial_{y}}}
\def\dxx{{\partial_{xx}}}
\def\dxy{{\partial_{xy}}}
\def\dyy{{\partial_{yy}}}
\def\dtt{{\partial^2_{t}}}

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\beqq{\begin{equation*}}
\def\eeqq{\end{equation*}}


\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\bigabs}[1]{\big|#1\big|}
\providecommand{\Bigabs}[1]{\Big|#1\Big|}
\providecommand{\Abs}[1]{\left\lvert#1\right\rvert}

\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\bignorm}[1]{\big\|#1\big\|}
\providecommand{\Bignorm}[1]{\Big\|#1\Big\|}
\providecommand{\Norm}[1]{\left\lVert#1\right\rVert}

\def\tb{\hbox{$\|\kern -.09em |$}}
\def\bigtb{\hbox{$\big\|\kern -.09em \big|$}}
\def\Bigtb{\hbox{$\Big\|\kern -.09em \Big|$}}

\providecommand{\tnorm}[1]{\tb#1\tb}
\providecommand{\bigtnorm}[1]{\bigtb#1\bigtb}
\providecommand{\Bigtnorm}[1]{\Bigtb#1\Bigtb}

\providecommand{\sprod}[2]{\langle#1,#2\rangle}
\providecommand{\bigsprod}[2]{\big\langle#1,#2\big\rangle}
\providecommand{\Bigsprod}[2]{\Big\langle#1,#2\Big\rangle}
\providecommand{\ssprod}[2]{\llangle#1,#2\rrangle}

\providecommand{\average}[1]{\{\!\!\{#1\}\!\!\}}
\providecommand{\jump}[1]{[\![#1]\!]}

    % \usepackage{stmaryrd}
    %  \llbracket     1 \rrbracket       \quad
    %  \llparenthesis 2 \rrparenthesis   \quad
    %  \llceil        3 \rrceil          \quad
    %  \llfloor       4 \rrfloor         \quad

\providecommand{\range}[2]{\llbracket #1, #2 \rrbracket}
\providecommand{\Range}[2]{\left\llbracket #1, #2 \right\rrbracket}




\newcommand\blue[1]{{\color{blue} #1}}
\newcommand\purple[1]{{\color{purple} #1}}

\providecommand{\note}[1]{{\bf [note: #1]}}
\providecommand{\todo}[1]{{\bf To do}: {\em #1 }}
\providecommand{\question}[1]{{\bf Question}: {#1}}
\def\blankfirst{\phantom{V^0} }
\def\blanksecond{\phantom{ \{ } } %\hspace*{-5pt}}
\def\bbb{\phantom{\big|} }
\def\bBb{\phantom{\Big|} }


\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\supp}{supp}

\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\gap}{gap}

\newcommand{\Curl}{\nabla \times}
\newcommand{\Grad}{\boldsymbol{\nabla}}
\newcommand{\Hcurl}{{H}(\mbox{curl}, \Omega)}


\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\rg}{range}
\DeclareMathOperator{\Dom}{Dom}

\DeclareMathOperator{\tbcurlh}{\widetilde \bcurl_{\it h}}
\DeclareMathOperator{\tcurlh}{\widetilde \curl_{\it h}}
\DeclareMathOperator{\bcurlh}{\bcurl_{\it h}}
\DeclareMathOperator{\curlh}{\curl_{\it h}}
\DeclareMathOperator{\tcurlha}{\widetilde \curl_{\it h}^{\it a}}

\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\bcurl}{{\bf curl}}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\bgrad}{{\bf grad}}

\DeclareMathOperator{\tgrad}{\widetilde \grad}
\DeclareMathOperator{\tcurl}{\widetilde \curl}
\DeclareMathOperator{\tDiv}{\widetilde \Div}

% black-board sans serif
% \mathbb require \usepackage ??  [bbgreekl]{mathbbol} of {upgreek} ??
\newcommand{\mat}[1]{\mathbb{#1}}
\def\matd{\mathbb{d}}
\def\matr{\mathbb{r}}
\def\matA{\mathbb{A}}
\def\matB{\mathbb{B}}
\def\matC{\mathbb{C}}
\def\matD{\mathbb{D}}
\def\matF{\mathbb{F}}
\def\matG{\mathbb{G}}
\def\matH{\mathbb{H}}
\def\matI{\mathbb{I}}
\def\matJ{\mathbb{J}}
\def\matK{\mathbb{K}}
\def\matL{\mathbb{L}}
\def\matM{\mathbb{M}}
\def\matN{\mathbb{N}}
\def\matO{\mathbb{O}}
\def\matP{\mathbb{P}}
\def\matR{\mathbb{R}}
\def\matS{\mathbb{S}}
\def\matT{\mathbb{T}}
\def\matW{\mathbb{W}}
\def\matX{\mathbb{X}}
\def\matZ{\mathbb{Z}}
\def\matLambda{\mathbb{\Lambda}}

% arrays of stacked quantities (dim = numerical parameter)
\newcommand{\arr}[1]{{\bs{\mathsf{#1}}}}
\newcommand\arre{{\bs{\mathsf{e}}}}
\newcommand\arrg{{\bs{\mathsf{g}}}}
\newcommand\arrB{{\bs{\mathsf{B}}}}
\newcommand\arrD{{\bs{\mathsf{D}}}}
\newcommand\arrE{{\bs{\mathsf{E}}}}
\newcommand\arrJ{{\bs{\mathsf{J}}}}
\newcommand\arrU{{\bs{\mathsf{U}}}}
\newcommand\arrV{{\bs{\mathsf{V}}}}
\newcommand\arrW{{\bs{\mathsf{W}}}}
\newcommand\arrX{{\bs{\mathsf{X}}}}
\newcommand\arrY{{\bs{\mathsf{Y}}}}
\newcommand\arrZ{{\bs{\mathsf{Z}}}}
\newcommand\arrLambda{{\bs{\mathsf{\Lambda}}}}
\newcommand\arrsigma{{\bs{\mathsf{\sigma}}}}
\newcommand\arrbeta{{\bs{\mathsf{\beta}}}}

\newcommand\uvec{{\be}}

\usepackage{mathrsfs}
\def\scrc{\mathscr{c}}
\def\scre{\mathscr{e}}
\def\scrf{\mathscr{f}}
\def\scrC{\mathscr{C}}
\def\scrE{\mathscr{E}}
\def\scrF{\mathscr{F}}
\def\scrP{\mathscr{P}}
\def\scrV{\mathscr{V}}

% grid nodes, edges, faces and cells
\newcommand\ttc{{\mathtt{c}}}
\newcommand\tte{{\mathtt{e}}}
\newcommand\ttf{{\mathtt{f}}}
\newcommand\ttg{{\mathtt{g}}}
\newcommand\ttj{{\mathtt{j}}}
\newcommand\ttn{{\mathtt{n}}}
\newcommand\ttx{{\mathtt{x}}}

\newcommand\ttC{{\mathtt{C}}}
\newcommand\ttE{{\mathtt{E}}}
\newcommand\ttF{{\mathtt{F}}}
\newcommand\ttG{{\mathtt{G}}}
\newcommand\ttN{{\mathtt{N}}}


\newcommand\gx{\bx}
%\newcommand\gx{{\bf{\texttt{x}}}}
% \def\gx{\bs{\ttx}}  % grid x



% interior products, continuous and discrete
\newcommand{\ip}[2]{i^{#1}_{#2}}
\newcommand{\tip}[2]{\tilde \imath^{#1}_{#2}}
\newcommand{\hiph}[2]{\hat \imath^{#1}_{h,#2}}
\newcommand{\iph}[2]{i^{#1}_{h,#2}}
\newcommand{\tiph}[2]{\tilde \imath^{#1}_{h,#2}}
% alternate notation:
%\newcommand{\ip}[2]{\imath^{#1}_{\uvec_{#2}}}
%\newcommand{\iph}[2]{I^{#1}_{h,\uvec_{#2}}}

